Formal Lagrangian Operad

Given a symplectic manifold $M$, we may define an operad structure on the the spaces $\op^k$ of the Lagrangian submanifolds of $(\bar{M})^k\times M$ via symplectic reduction. If $M$ is also a symplectic groupoid, then its multiplication space is an associative product in this operad. Following this idea, we provide a deformation theory for symplectic groupoids analog to the deformation theory of algebras. It turns out that the semi-classical part of Kontsevich's deformation of $C^\infty(\R^d)$ is a deformation of the trivial symplectic groupoid structure of $T^*\R^d$.

==> draws/RT-1.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/RT-1.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3572,2095)(906,-2054)
\end{picture}


==> draws/RT-2.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/RT-2.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3572,2095)(906,-2054)
\end{picture}


==> draws/RT-3.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/RT-3.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3572,2095)(906,-2054)
\end{picture}

